Branch Target Buffer Reverse Engineering on Arm

The Branch Target Buffer (BTB) plays a critical role in efficient CPU branch prediction. Understanding the design and implementation of the BTB provides valuable insights for both compiler design and the mitigation of hardware attacks such as Spectre. However, the proprietary nature of dominant CPUs, such as those from Intel, AMD, Apple, and Qualcomm, means that specific BTB implementation details are not publicly available. To address this limitation, several previous works have successfully reverse-engineered BTB information, including capacity and associativity, primarily targeting Intel's x86 processors. However, to our best knowledge, no research has attempted to reverse-engineer and expose the BTB implementation of ARM processors. This project aims to fill the gap by exploring the BTB of ARM processors. Specifically, we investigate whether existing reverse-engineering techniques developed for Intel BTB can be adapted for ARM. We reproduce the x86 methodology and identify specific PMU events for ARM to facilitate the reverse engineering process. In our experiment, we investigated our ARM CPU, i.e., the quad-core Cortex-A72 of the Raspberry Pi 4B. Our results show that the BTB capacity is 4K, the set index starts from the 5th bit and ends with the 15th bit of the PC (11 bits in total), and there are 2 ways in each set. The source code can be find at https://github.com/stefan1wan/BTB_ARM_RE.

==> z.backup.tex <==
\subsection{How to add Lists}

You can make lists with automatic numbering \dots

\begin{enumerate}
\item Like this,
\item and like this.
\end{enumerate}
\dots or bullet points \dots


\begin{itemize}
\item Like this,
\item and like this.
\end{itemize}

\subsection{How to write Mathematics}

\LaTeX{} is great at typesetting mathematics. Let $X_1, X_2, \ldots, X_n$ be a sequence of independent and identically distributed random variables with $\text{E}[X_i] = \mu$ and $\text{Var}[X_i] = \sigma^2 < \infty$, and let
\[S_n = \frac{X_1 + X_2 + \cdots + X_n}{n}
      = \frac{1}{n}\sum_{i}^{n} X_i\]
denote their mean. Then as $n$ approaches infinity, the random variables $\sqrt{n}(S_n - \mu)$ converge in distribution to a normal $\mathcal{N}(0, \sigma^2)$.

    % \begin{figure}
    %     \centering
    %     \includegraphics[width=0.3\textwidth]{figure/capacity_x86.png}
    %     \caption{\label{fig:capacity_x86}Misprediction Rate on Skylake CPU}
    % \end{figure}
      % \begin{figure}
    %     \centering
    %     \includegraphics[width=0.3\textwidth]{figure/capacity_arm.png}
    %     \caption{\label{fig:capacity_arm}Misprediction Rate on Kunpeng 920 CPU}
    % \end{figure}


    % Here, we will explore if the frontend bottleneck is related to the deficiency of BTB capacity.
% The frontend bottleneck is closely related to whether the BTB is large enough to hold all the branch targets. [in the body === Use the number or figure of ISA wars. To connect the BTB MPKI to CPU frontend bottle neck. It's clear that if there is a higher MPKI, the frontend bottleneck is more significant.=> only mention two data, .]

% Conclusion: In 5 cloud server workloads, 2 will be benefited by a larger BTB capacity; 3 will not be benefited. If the architecture servers will be benefited by larger BTB capacity is depends on other considerations, like the percentage of each workloads. 
(The bottleneck of CPU frontend will be caused by:   )
% introduction could be extented from abstract;
(1) background => Branch Target Buffer(BTB) is crucial to the Branch Predict Unit(BPU) to predict the next branch. which will help CPU to fetch instrctions in advance and provide enough uops to the backend. 
(2) question =>  BTB capacity deficiency will cause frontend bottleneck thus lower the IPC of CPU. According to our measurement, the frontend bottleneck is range from xx\% to xx\%, the frontend is a bottleneck of CPU which executing cloud applications expecially for workload A and workload B. 
(3) our work =>
In this work, we try to confirm if the BTB capacity deficiency exists, which is that the BTB capacity is big engough to hold branches on cloud benchmarks. And if the BTB capacity deficiecny is related to the frontend bottleneck in modern CPU. 
(4) EXP => We choose cloudsuite as our investiment target, which is a popluar and representative cloud workload. By comparing the branch working sets, which we get from cache simulation for cloud workloads, and the BTB capacity, which we get from reverse engineering, we found their current BTB capacity is sufficient for most scenarios. 
(5) Conclusion=> The  BTB capacity deficiency exists in 2 out of the 5 cloud workloads of cloudsuite, which is close related to the frontend bottleneck for this workloads.

Our experiment platforms are Xeon Gold 6132 and Kunpeng 920. And there are x86 server CPU(Skylake), and Arm server CPU(Taishan) inside repectively. However, we could not find public documents of BTB capacity about Skylake-SP and Taishai V100. However, previous work have propose solutions about how to revesrse engineering it on Intel Pentium M \cite{btbrex86}. In this section, we reproduce the reverse engineering results on Skylake-SP. Besides, we reapply the same methodology on Arm v8, and get the BTB capacity and other information successfully. 

Previous work \cite{btbrex86} has explained the reverse engineering details of BTB on x86, including the capacity. Therefore, in this section, we will only introduce the reverse engineering process on Arm. Basicly, our tool is PMU events, especially there is an event called \textit{ARM\_PMU\_BR\_MIS\_PRED}. By counting its counters when executing a bunch of branches, we will know that if there is a mispredicted or not predicted branch \cite{arm2015armv8}. 


We count the above PMU events upon running our test gadget, which is explained in the following pseudocode. This gadget consists of fall-through unconditional indirect branches. We control the branch number B and the align distance N, where N is the gap(bytes) between two labels(or basic blocks). 
% By controlling B, we control how many branch targets in this piece of code and by controlling N, we 
%\begin{verbatim}

We count branch misprediction rates for different B and N.  For each test:  we first execute our test gadget 10 times to warm up the BTB;  secondly, we run the test gadget once and log the difference of the PMU event counter(C). Then the branch misprediction rate is C/B. By comparing and analyzing the misprediction rate of all B and N in a two-dimentional way, we could infer the BTB capacity of the BPU.

Since the BTB is also a kine of cache, its orgnization is similar to other kinds of caches\cite{btbrex86}. Assume there are S sets and each set has W ways, then the BTB entry capacity is $C=SxW$. We could see the related BTB bits of PC in figure \ref{fig:btbaddr}, the bits near the lower bits are used for set index and the bits near the higher bits are used for tags. 

    The misprediction rate from our reverse engineering of TaiShan V110 CPU is on figure \ref{fig:capacity_arm}.
    From figure \ref{fig:capacity_arm}, we could know that:

     \item The BTB set index starts from bit 5. Because when B goes from 3K to 7k, the misprediction rate is almost the same if N goes from 16 to 32 ($32=2^5$); but when B goes from 3K to 7k, the misprediction rate has a leap from 32 to 64 ($64=2^6$). Since when N is 32, the lower 5 bits is same for all PCs and when N is 64, the lower 6 bits is same for all PCs, its clearly that the 6th bit is included in the set index thus cause different targets fall in same BTB sets.
        
        \item The BTB entry size is 4096. Because when N is 32, the rate is 0.01 for 4K however 0.39 for 5K. By the way, there are still 40-50 branches not buffered by BTB. It may be introduced by timer interrupts.


        % todo: align with the result of uops splits.


% Among our workloads, Data Serving and Web Serving benefit from having
% more than 4 K entries BTB. Their sensitivity to BTB size is
% shown in \ref{table:BTB}. For the rest of the workloads, a 4 K entry
% BTB effectively captures the branch working set. We do not
% observe a distinguishable difference between x86 and ARM
% branch traces. Designing a more powerful branch prediction
% unit not only mitigates bad speculation stalls but also enables
% effective instruction prefetching to address the frontend stalls
% using an FDIP-based instruction prefetcher [56].

Based on our reverse enigeering results, the BTB capicity is 4K for both Skylake and TaiShan V110. And based on our results of cache simulation, when the BTB entry size is 4K, the workload Data Serving Web Serving has a relative high MPKI, which has about 9 or 5 branch target misses per 1000 instructions. Assume there are one fifth branch instructions in these 1000 instructions which is 200, these two workload are suffer from BTB capacity deficiency. For the rest of the workloads, 4K entry is enough for capturing the branch working set. 
